Dynamics-Aware Quality-Diversity for Efficient Learning of Skill Repertoires

Quality-Diversity (QD) algorithms are powerful exploration algorithms that allow robots to discover large repertoires of diverse and high-performing skills. However, QD algorithms are sample inefficient and require millions of evaluations. In this paper, we propose Dynamics-Aware Quality-Diversity (DA-QD), a framework to improve the sample efficiency of QD algorithms through the use of dynamics models. We also show how DA-QD can then be used for continual acquisition of new skill repertoires. To do so, we incrementally train a deep dynamics model from experience obtained when performing skill discovery using QD. We can then perform QD exploration in imagination with an imagined skill repertoire. We evaluate our approach on three robotic experiments. First, our experiments show DA-QD is 20 times more sample efficient than existing QD approaches for skill discovery. Second, we demonstrate learning an entirely new skill repertoire in imagination to perform zero-shot learning. Finally, we show how DA-QD is useful and effective for solving a long horizon navigation task and for damage adaptation in the real world. Videos and source code are available at: https://sites.google.com/view/da-qd.

==> psuedocode.tex <==

\algnewcommand{\LeftComment}[1]{\State \(\triangleright\) #1}

\begin{algorithm}[ht!]
  \small
% \SetAlgoLined
% \DontPrintSemicolon

\caption{\algonamefull{} (\algoname{})}
  \newcommand\algorithmicitemindent{\hspace*{\algorithmicindent}\hspace*{\algorithmicindent}}
\label{algo:mb-qd}
  \begin{algorithmic}[1]

 \State{Initialize repertoire $\archivereal$ (to $\varnothing)$, imagined repertoire $\archivesynthetic$ (to $\varnothing$), dynamics model $\dynamicsmodel$, and replay buffer $\replaybuffer$ (to $\varnothing)$}
 \\
 \While{maximum number of evaluations not reached}
 \\
  \If{first iteration} \Comment{\textit{Generate random policies at first iteration.}}
      \State{$\batchpoliciesrealmutated \leftarrow$ random\_parameters()}

  \Else
        \State{$\batchpoliciesreal \leftarrow$ select($\archivereal$) \Comment{\textit{Selecting $b$ policies from repertoire $\archivereal$ (section~\ref{sec:background}).}}}
        \State{$\batchpoliciesrealmutated \leftarrow$ variation\_operators($\batchpoliciesreal$) \Comment{\textit{Apply variations to parameters $\param{i}$.}}}
    \EndIf
    \\
    
    \LeftComment{\textit{Performing QD Exploration in Imagination (section~\ref{sec:methods-qd_exploration_imag})}}
  \While{model stopping criterion is False}
  
    \State{$(\widetilde{\skilldescriptor_i}, \widetilde{\reward_i})_{i\in\left[1,b\right]} \leftarrow$ imagined\_rollouts($\batchpoliciesrealmutated$) using $\dynamicsmodel$ \Comment{\textit{Evaluate using dynamics model. }}}
    
    \State{$\archivesynthetic$ $\leftarrow$ model\_condition($\batchpoliciesrealmutated,\archivesynthetic$) \Comment{\textit{Add $\policyrealmutated{i}$ to $\archivesynthetic$ depending on $\widetilde{\reward_i}$ and novelty of $\widetilde{\skilldescriptor_i}$.}}}
    
    \If{model stopping criterion is False} \Comment{\textit{Continue performing QD exploration in imagination.}}
    
        \State{$\batchpoliciesreal \leftarrow$ select($\archivesynthetic$) \Comment{\textit{Selecting $b$ policies from imaginary repertoire $\archivesynthetic$.}}}
        
        \State{$\batchpoliciesrealmutated \leftarrow$ variation\_operators($\batchpoliciesreal$)}
        
    \EndIf
  \EndWhile
  
\\
\LeftComment{\textit{Acting in the Environment (section~\ref{sec:methods-acting_in_env})}}
  \State{$\batchpoliciesreal[N]{}$ $\leftarrow$ select($\archivesynthetic$) \Comment{\textit{Selecting $N$ policies from imaginary repertoire $\archivesynthetic$ to be evaluated.}}}
  
  \State{($\skilldescriptor_i, \reward_i)_{i\in\left[1,N\right]}$, transitions $\leftarrow$ evaluation($\batchpoliciesreal[N]{}$) \Comment{\textit{Evaluate in environment; get transitions.}}}
  \State{$\replaybuffer \leftarrow$ add\_to\_replay\_buffer(transitions, $\replaybuffer$)}
  
  \State{$\archivereal$ $\leftarrow$ repertoire\_condition($\batchpoliciesreal[N]{}, \archivereal$) \Comment{\textit{Add $\policyreal{i}$ to $\archivereal$ depending on $\reward_i$ and novelty of $\skilldescriptor_i$.}}}
  
  \State{$\archivesynthetic$ $\leftarrow$ synchronise\_repertoires($\archivereal$, $\archivesynthetic$)
  \Comment{\textit{Erase content of $\archivesynthetic$ and replace it with the content from $\archivereal$.}}}
  
  
  \\
  \LeftComment{\textit{Learning Dynamics Models (section~\ref{sec:methods-dyn_model})}}
  \State{Update $\dynamicsmodel$ using $\replaybuffer$ \Comment{\textit{Train dynamics model with transitions collected in replay buffer.}}}
  
  \EndWhile
  \\
  \State \Return $\archivereal$
  \end{algorithmic}
\end{algorithm}

==> tables/table_ablation_selection_acquisition.tex <==

\begin{table*}[t]
\small
\centering
\begin{threeparttable}
\begin{tabular}{ lrrrr } 
 \toprule
 Algorithm & Evaluations & Best Return & Mean Return  & Repertoire Size \\
 \midrule 
 \algoname{} & $2{,}705\tnote{1}$ & $0.471$ & $0.191$ & $838$\\ 
%   \addlinespace
 Vanilla QD (Equivalent) & $3{,}000$ & $0.353$ & $0.068 $ & $662 $ \\
 Vanilla QD (Upper Baseline) & $100{,}000$ & $0.497$ & $0.177$ & $3{,}225$ \\ 
 %Vanilla QD (Equivalent) & $10{,}000$ & $0.41\pm0.027$ & $0.097\pm0.005$ & $1{,}320\pm 48$ \\
 %Vanilla QD (Equivalent) & $3{,}500$ & $0.37 \pm 0.04$ & $0.072 \pm 0.008$ & $744 \pm 28$ \\
 %\algoname{} (Direct Add) & $2,575 \pm 359$ & $0.47 \pm 0.07$ & $0.13 \pm 0.06$ & $2575 \pm 359$ \\ 
 \midrule
 \algoname{} (20-shot) & 20 & $0.33$ & $0.11$ & - \\ \algoname{} (15-shot) & 15 & $0.31$ & $0.11$ & - \\
 \algoname{} (10-shot) & 10 & $0.25$ & $0.11$ & - \\
 \algoname{} (5-shot) & 5 & $0.22$ & $0.10$ & -\\
 \algoname{} (2-shot) & 2 & $0.16$ & $0.11$ & -\\
 \algoname{} (Zero-shot) & 1 & $0.16$ & - & -\\ 
 \bottomrule
\end{tabular}
\end{threeparttable}
\vspace{2mm}
\caption{
Performance results obtained for \algoname{} in new skill acquisition, and for its equivalent and upper QD baselines.
%
The zero-shot and few-shot performance of \algoname{} are also displayed.
%
For each variant, we generated 10 different repertoires from independent replications and report the median.
%
%We report the medians of the results obtained from those replications.
\vspace{-8mm}
} \label{table:continual-ablation-results}
\end{table*}
